CPG-ACTOR: Reinforcement Learning for Central Pattern Generators

Central Pattern Generators (CPGs) have several properties desirable for locomotion: they generate smooth trajectories, are robust to perturbations and are simple to implement. Although conceptually promising, we argue that the full potential of CPGs has so far been limited by insufficient sensory-feedback information. This paper proposes a new methodology that allows tuning CPG controllers through gradient-based optimization in a Reinforcement Learning (RL) setting. To the best of our knowledge, this is the first time CPGs have been trained in conjunction with a MultilayerPerceptron (MLP) network in a Deep-RL context. In particular, we show how CPGs can directly be integrated as the Actor in an Actor-Critic formulation. Additionally, we demonstrate how this change permits us to integrate highly non-linear feedback directly from sensory perception to reshape the oscillators' dynamics. Our results on a locomotion task using a single-leg hopper demonstrate that explicitly using the CPG as the Actor rather than as part of the environment results in a significant increase in the reward gained over time (6x more) compared with previous approaches. Furthermore, we show that our method without feedback reproduces results similar to prior work with feedback. Finally, we demonstrate how our closed-loop CPG progressively improves the hopping behaviour for longer training epochs relying only on basic reward functions.

==> old_methodology.tex <==
\subsection{CPGs differentiable formulation}\label{cpg_differentiable_formulation}

As mentioned in \cref{introduction}, historically \glspl{cpg} have been tuned with \gls{ga}, \gls{pso} or by hand.
Population-based algorithms spawn many instances of controllers that act on the environment; performances for each of them are measured and based on them the best individuals are selected.

Parallel implementations of \gls{rl} algorithms spawn the same policy $\pi_{\theta}$ on parallel instances of the same robot to gather quickly more experiences.
Once the interactions with the simulation environment ends, the observations are fetched in batches and used to update the actor and the critic.

Since the update is based on gradient descent algorithms, such as Adam \cite{Diederik2015}, the implementation of \glspl{cpg} must be differentiable. 
Being \glspl{cpg} a network of neurons, organizing \cref{eqn:cpg_hopf} into tensor operations is the most natural solution.

\subsection{Hopf Oscillators}

The equation of the single Hopf oscillator is given in \cref{eqn:cpg_hopf}.

\begin{align}
    \label{eqn:cpg_hopf}
    \begin{split}
        \dot \theta_i = 2\pi\nu_i + \sum_{j} r_jw_{ij}\sin(\theta_j - \theta_i - \phi_{ij}) + \theta_f
        \\
        \ddot r_i =  a_i(\frac{a_i}{4}(R_i - r_i) - \dot r_i) + r_f
        \\
        x_i = r_i\cos(\theta_i)
    \end{split}
\end{align}
%
where $\theta_i$ and $r_i$ are the state variables representing the phase and the amplitude of oscillator $i$ respectively, $\nu_i$ and $R_i$ determine its intrinsic frequency and amplitude, and $a_i$ is a positive constant governing the amplitude dynamics.
Couplings between oscillators are defined by the weights $w_{ij}$ and phase $\phi_{ij}$.
The signal $x_i$ represents the burst produced by the oscillatory center used as reference by the motors.
While $\theta_{f}$ and $r_{f}$ are the feedback components provided by the \gls{mlp} network.

The control command $d_i$ is included in $\nu_i$ as illustrated in supplementary material of \cite{ijspeert2007}.

Note, in order to apply batch updates and gradient estimation in the actor-critic framework, care has to be taken for the implementation of the tensor operations.
% However, differently from previous applications \cite{ajallooeian2013}, the tensor operations have to take care of the batches used during the updates. 
% This additional complexity, in conjunction with the recurrent nature of \glspl{cpg}, required several iterations before reaching the final formulation.

\subsection{How to deal with the recurrent terms}\label{how_to_deal_with_recurrent_state}

Stateless networks, such as \glspl{mlp}, do not need any information from the previous state to compute the next step and the backpropagation procedure is faster and straightforward.

Otherwise, \glspl{rnn} are stateful networks, which means that the state from the previous time-step is needed to compute the following step output, as consequence they require more time  and a specific procedure to be trained. 
\glspl{rnn} rely on \gls{bptt}, \cref{fig:backprop_rnn}, which is a gradient-based technique specifically designed to train stateful networks. 

It consists in unfolding a recurrent neural network in time: the unfolded network contains $t$ inputs and outputs, one for each time step.
The transition from an input $x_t$ to an output $y_t$ depends on three different matrices: $W_{xh}$ determines the transition between the $x_t$ and the hidden state $h$, $W_{hy}$ regulates the transformation from $h_t$ to $y_t$ and lastly $W_{hh}$ governs the evolution between two hidden states. All the matrices $W_{xh}$, $W_{hy}$, $W_{hh}$ are initially unknown and tuned during the optimization.

\begin{figure}[h!]
    \centering
        
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/rnn_backprop.png}
        \caption{}
        \vspace{5pt}
        \label{fig:backprop_rnn}
    \end{subfigure}
    
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/cpg_backprop.png}
        \caption{}
        \vspace{5pt}
        \label{fig:backprop_cpg}
    \end{subfigure}
    
    \caption{The images above show the difference between back-propagation for classic \glspl{rnn} (\ref{fig:backprop_rnn}) and \glspl{cpg} (\ref{fig:backprop_cpg}). In particular to train \glspl{rnn} the matrices $W_{xh}$, $W_{hy}$, $W_{hh}$ have to be tuned, where $W_{hh}$ regulates the evolution between two \textit{hidden states}. Instead for \glspl{cpg} only the parameters in $\dot \theta_i$ and $\ddot r_i$ (\cref{eqn:cpg_hopf}) need tuning, while the evolution of the \textit{hidden state} is determined by \cref{eqn:cpg_hidden_state_evolution}.}
    \label{fig:backprop}
\end{figure}

Due to its complexity, the recurrent nature of \glspl{cpg} discouraged previous researches to pursue this direction.

Undeniably \glspl{cpg} have a recurrent nature, but the transition between consecutive hidden states is determined a priori using \cref{eqn:cpg_hidden_state_evolution} without the need of tuning $W_{hh}$, as \glspl{rnn} do.
However, \glspl{cpg} require storing the previous hidden state until the next step.

\begin{equation}
    \label{eqn:cpg_hidden_state_evolution}
    \begin{split}
        \theta = \theta_{old} + (\dot \theta_{old} + \dot \theta) \frac{dt}{2}
        \\
        \dot r = \dot r_{old} + (\ddot r_{old} + \ddot r) \frac{dt}{2}
        \\
        r = r_{old} + (\dot r_{old} + \dot r) \frac{dt}{2}
    \end{split}
\end{equation}

The observation above leads to two significant consequences: firstly \glspl{cpg} do not have to be unrolled to be trained, since given the previous state and the new input, the output is fully determined and secondly eliminating $W_{hh}$ has the additional benefit of entirely excluding any gradient explosion or vanishing during training; both points are illustrated in \cref{fig:backprop_cpg}. 

Therefore, \glspl{cpg} can be framed as stateless network on condition that the previous state is passed as an input of the system.
This addresses both the limitations mentioned in \cite{Fukunaga2004}: \glspl{cpg} are recurrent networks and \glspl{rnn} take a long time to train.

\begin{figure*}[ht!]
    \centering

    \begin{subfigure}{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cpg_params_histogram.png}
        \caption{}
        \label{fig:cpg_param_training}
    \end{subfigure}
    ~
    \begin{subfigure}{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cpg_mlp_feedback_weight.png}
        \caption{}
        \label{fig:mlp_weight_feedback}
    \end{subfigure}
    ~
    \begin{subfigure}{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cpg_mlp_feedback_bias.png}
        \caption{}
        \label{fig:mlp_bias_feedback}
    \end{subfigure}
    
    \caption{The set of images above show how the distributions of \glspl{cpg} parameters (\cref{fig:cpg_param_training}), weights (\cref{fig:mlp_weight_feedback}) and biases (\cref{fig:mlp_bias_feedback}) of the output layer of \gls{mlp} network change during training. As explained in \cref{cpg_differentiable_formulation} they have been trained in conjunction resorting on gradient-based optimisation: the gradient flows through all of the components simultaneously.}
    \label{fig:parameters_under_training}
\end{figure*}

\subsection{Proximal Policy Optimization}
\Gls{ppo} \cite{Schulman2017} is a model-free, online, on-policy, policy-gradient \gls{rl} method and it is nowadays considered as a state-of-the-art actor-critic method.
It takes inspiration from \gls{trpo} \cite{Schulman2017} and proposes a loss that approximate the KL-divergence, as shown below.
% It is considered as a state-of-the-art actor-critic method, and we will thus use it for training our \gls{cpg}-actor-critic formulation.

In \gls{trpo} \cite{Schulman2015}, an objective function (the “surrogate” objective) is maximized subject to a constraint on the size of the policy update:

\begin{equation}
    \label{eqn:trpo_objective}
    \begin{split}
        \max_{\theta} \; \hat{\mathbb{E}}_t\left[\frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_{old}(a\,|\,s)}\hat{A}_t\right]
        \\
        subject\:to\;\;\;\hat{\mathbb{E}}_t\left[KL[\theta_{old}(\cdot,\:s_t), \theta(\cdot,\:s_t)]\right] \le \delta
    \end{split}
\end{equation}

Alternatively \gls{trpo} can be solved using the KL-divergence as penalty, hence removing the constraint:

\begin{equation}
    \label{eqn:trpo_objective_penalty}
    \begin{split}
        \max_{\theta} \; \hat{\mathbb{E}}_t\left[\frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_{old}(a\,|\,s)}\hat{A}_t\right] - \beta\left[KL[\theta_{old}(\cdot,\:s_t), \theta(\cdot,\:s_t)]\right]
    \end{split}
\end{equation}

\Gls{ppo} introduces a new objective, which approximate the KL-divergence, simplifying the implementation, the computations and improving the overall performances:

\begin{equation}
    \label{eqn:ppo_objective}
    \begin{split}
        considering\;\;\;r_t(\theta) = \frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_{old}(a\,|\,s)}
        \\
        L^{PPO} = \hat{\mathbb{E}}_t\left[\min(r_t(\theta)\hat{A}_t, clip(r_t(\theta), 1-\epsilon, 1+\epsilon)\hat{A}_t)\right]
    \end{split}
\end{equation}

==> recycling.tex <==
% Old snippets removed from main manuscript


%\begin{equation}
%    \label{eqn:cpg_hopf}
%    \begin{array}{lcl}
%        \dot \theta_i = 2\pi\nu_i(d_i) + \zeta_i + \xi_i
%        \\
%        \zeta_i = \sum_{j} r_j w_{ij} \sin(\theta_j - \theta_i - \phi_{ij})
%        \\
%        \ddot r_i =  a_i(\frac{a_i}{4}(\rho_i(d_i) - r_i) - \dot r_i) + \kappa_i
%        \\
%        x_i = r_i\cos(\theta_i)
%    \end{array}
%\end{equation}

%\subsection{Proximal Policy Optimization}
%\Gls{ppo} \cite{Schulman2017} is a model-free, on-policy, policy-gradient \gls{rl} method and it is nowadays considered as a state-of-the-art actor-critic method.
%It takes inspiration from \gls{trpo} \cite{Schulman2017} and proposes a loss that approximates the KL-divergence.

% It is considered as a state-of-the-art actor-critic method, and we will thus use it for training our \gls{cpg}-actor-critic formulation.

%In \gls{trpo} \cite{Schulman2015}, an objective function (the “surrogate” objective) is maximized subject to a constraint on the size of the policy update:

%\begin{equation}
%    \label{eqn:trpo_objective}
%    \begin{split}
%        \max_{\theta} \; \hat{\mathbb{E}}_t\left[\frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_{old}(a\,|\,s)}\hat{A}_t\right]
%        \\
%        \text{s.t.}\;\;\;\hat{\mathbb{E}}_t\left[KL[\theta_{old}%(\cdot,\:s_t), \theta(\cdot,\:s_t)]\right] \le \delta
%    \end{split}
%\end{equation}
%
%Alternatively \gls{trpo} can be solved using the KL-divergence as penalty, hence removing the constraint:
%
%\begin{equation}
%    \label{eqn:trpo_objective_penalty}
%    \begin{split}
%        \max_{\theta} \; %\hat{\mathbb{E}}_t\left[\frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_%{old}(a\,|\,s)}\hat{A}_t\right] - %\beta\left[KL[\theta_{old}(\cdot,\:s_t), %\theta(\cdot,\:s_t)]\right]
%    \end{split}
%\end{equation}
%
%\Gls{ppo} introduces a new objective, which approximates the KL-divergence, simplifying the implementation, the computations and improving the overall performances:
%
%\begin{equation}
%    \label{eqn:ppo_objective}
%    \begin{split}
%text{considering}\;\;\;r_t(\theta) = \frac{\pi_\theta(a\,|\,s)}{{\pi_\theta}_{old}(a\,|\,s)}
%        \\
%        L^{PPO} = %\hat{\mathbb{E}}_t\left[\min(r_t(\theta)\hat{A}_t, %clip(r_t(\theta), 1-\epsilon, 1+\epsilon)\hat{A}_t)\right]
%    \end{split}
%\end{equation}

%\section{Practical considerations}

%Before adopting \gls{ppo} to train \glspl{cpg} several modifications are needed to make them compatible with existing implementations of the algorithm. 
%The \glspl{cpg}, with the set of variations required to make them fully functional is what we call \gls{cpg}-Actor and it is described in details in the sections below.

%\subsubsection{Remembering the previous hidden state}

%As we discussed in \cref{sec:how_to_deal_with_recurrent_state}, the \glspl{cpg} can be framed in a stateless formulation, as far as the previous hidden state is part of the inputs to the controller.

%To do that,  the \textit{hidden state} is concatenated with the actions and sent from the controller to the environment, at the first cycle the actions are set to zero.

%Upon receipt, the environment splits the action into \textit{real action}, the reference trajectory computed by \glspl{cpg}, and \textit{hidden state}.
%The \textit{real action} are used to control the robot and its interaction with the environment in simulation produces new observations, that are then concatenated with the \textit{hidden state} and sent back to the controller.

%The controller splits the observations into \textit{real observations} and \textit{previous hidden state}, it uses them to compute the new output and the new hidden state. 
%%\subsubsection{Action dim, observation dim and their boundaries}

%Following the integration of the \textit{hidden state}, action and observation change.
%OpenAI set some guidelines on the creation of new environments, among these it is required to provide \textit{action dim}, \textit{observation dim}, \textit{action space} and \textit{observation space}.
%They respectively are the dimension of the actions, of the observations and the inferior and superior boundaries for each of the actions and observations.
%Regarding the boundaries on the actions, it is important to bound only the fields corresponding to the \textit{real actions} and leave unbounded the ones related to the \textit{hidden state} to allow its free evolution over time.

%\subsubsection{Sampling from distributions}\label{sampling_from_distribution}

%The actions that \gls{ppo} sends to the environment are sampled from a normal distribution to improve exploration: the $mean$ is the output of the controller, while the $std$ is learned.

%Since the output of \gls{cpg}-Actor is the concatenation of the \textit{hidden state} and the \textit{real actions}, before sampling happens it is vital to define the $hidden\:state\:std = 0$. 
%Otherwise the \textit{hidden state} received by the environment will be different from the original.
%Moreover, the $action\:std$ is usually initialised to $1$ which corresponds to $\approx\left[-60\si{\degree},+60\si{\degree}\right]$ and reducing it forces the policy to rely more on \glspl{cpg}' output and less on random sampling from the distribution.

%\section{Discussion} \label{sec:discussion}
%The main benefit of the proposed approach is that it provides a fully differentiable pipeline for training \gls{cpg}-based controllers.
%The development of this tool allows us to train \glspl{cpg} with \gls{rl} which has been recently demonstrated to have impressive performance. Additionally, this setup enables us to improve \glspl{cpg}' capabilities of understanding the surrounding environment.
%It is further possible to introduce \glspl{nn} in the same pipeline, since they all rely on gradient-based optimisation.



% % L.C. proposed the theoretical base of the approach.
% % D.D.M proposed the \gls{cpg} differential formulation. 
% % L.C. upgraded the \gls{cpg} differential formulation to process batches.
% % L.C and S.G. worked on the \gls{rl} environment.
% % W.M. proposed modifications to the pyBullet environment.
% % L.C. wrote the control software Cpg-Actor.
% % S.G. proposed modifications to Cpg-Actor.
% % L.C. implemented previous baseline, carried out the experiments and produced the results.
% % L.C. took the lead in writing the manuscript.
% % D.D.M., S.G. and W.M. provided critical feedback and helped shape the manuscript.
% % I.H. provided critical feedback, helped shape the manuscript and provided funding.

% % I would like to thank again Alex, David and Sid, not only colleagues but also friends, for their support.


